Emotion Analysis of Social Media Bangla Text and Its Impact on Identifying the Author's Gender

The Gender Identification (GI) problem is concerned with determining the gender of the author from a given text. It has numerous applications in different fields like forensics, literature, security, marketing, trade, etc. Due to its importance, researchers have put extensive efforts into identifying gender from the text for different languages. Unfortunately, the same statement is not true for the Bangla language despite its being the 7th most spoken language in the world. In this work, we explore Gender Identification from Social media Bangla Text. Specially, we consider two approaches for feature extraction. The first one is Bag-Of-Words(BOW) approach and another one is based on computing features from sentiment and emotions. There is a common stereotype that female authors write in a more emotional way than male authors. One goal of this work is to validate this stereotype for the Bangla language.

==> Tex_Code/3.method/A.dataset.temp.tex <==
\subsection{Dataset Creation}\label{AA}
We extract facebook posts from five different facebook groups consisting of authenticated members, using Facebook Graph API version 3.0. Some annotated sample posts shown in Table II. We collect facebook posts with posts author names and separately collect the the members list using Graph API. We manually label the members as Male and Female. Then we assign the author gender by cross multiplying the posts data with author name and labeled members list.

We do not use user API to get user gender since we do not have user level permission. For labeling members we tokenize the unique member names and we manually assign the Male, Female and Common to these tokens. For example from member name "Sajid Hasan" we get tokens "Sajid" and "Hasan" to which we assign "Male" and "Common" labels. On the other hand, from member name "Sanjida Hasan" we get tokens "Sanjida" and "Hasan" to which we assign "Female" and "Common" labels. We collect 10,000 unique members name and we get 2000 Male token, 2500 Female token, 1500 common tokens. Then we get label for original members name from the assigned tokens.

==> Tex_Code/3.method/E.latex_advice.tex <==
\subsection{\LaTeX-Specific Advice}
Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

==> Tex_Code/3.method/F.mistakes.tex <==
\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

==> Tex_Code/3.method/G.authors.tex <==
\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

==> Tex_Code/3.method/H.headings.tex <==

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

==> Tex_Code/3.method/I.figures.tex <==
\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and  bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be  below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation ``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

==> Tex_Code/4.experiment/A.experimental.evaluation.tex <==
\subsection{Experimental Setup}
We have employed Python Keras framework with Tensorflow as a framework to implement deep learning models for training, tuning, and testing. We have also used Gensim package for word2vec model implementation. Scikit-learn package is used to implement traditional machine learning algorithms. Experimental evaluation was conducted on a machine with an Intel Core i7 processor with 1.8GHz clock speed and 8GB RAM. The machine has also an Nvidia GeForce MX150 with 2GB memory and therefore Tensorflow based experiments have fully utilized GPU instructions. Considerable speed can be achieved in Tensorflow based experiments by adding a GPU as shown in ~\cite{JMLR_speed_gpu}. 

==> Tex_Code/4.experiment/B.performance.evaluation.tex <==
\subsection{Performance Evaluation and Parameter Tuning}
We have studied the efficiency and scalability of our proposed methods by varying model architectures and feature set vectors. We have measured performance of recurrent neural network, LSTM model by generating word vector using stylometric feature method and using word2vec method. Moreover, we have evaluated the performance of different word2vec model by initializing embedding layer weights with them and consider both trainable and non-trainable weight matrix. Trainable weight matrix denotes that at the time of training, the embedding layer weights will be updated. Non-trainable weight matrix denotes  that the embedding layer weights will not be updated at the time of training.\endgraf 

We have used RMSprop optimizer and binary cross entropy as loss function. Epoch and batch size are the parameters of the Machine Learning algorithm LSTM. Epochs are the number of complete passes through the training dataset and batch size is the number of samples processed before the model is updated. Fig~\ref{fig:4_ii_accuracy} shows that the accuracy does not increase for training set after a certain epochs. It is also observed that the loss in the validation set increases also with an increase in epoch number. Therefore, the overfitting problem exists in our methods.  As a result, we set the epoch number to 5 in all experiments and use batch size 32. \endgraf


\begin{figure*}[!tbp]
       \centering
\begin{subfigure}[t]{0.45\textwidth}
\includegraphics[width=\textwidth]{Tex_Code/resource/image/4.1.png}
\caption{Accuracy} \label{fig:4_ii_a_accuracy}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.45\textwidth}
\includegraphics[width=\textwidth]{Tex_Code/resource/image/4.2.png}
\caption{Loss}
\label{fig:4_ii_b_accuracy} 
\end{subfigure}
\caption{Effect of Epoch in Accuracy and Loss}
  \label{fig:4_ii_accuracy}
\end{figure*}
 


We experiment with our model by running ten times for each configuration and calculate the average performance. The algorithm to experiement is given in ~\ref{alg:10_fold_cross_valid}. The accuracy and F1 score of the testing set is presented as our evaluation measure.

\begin{algorithm}
\caption{10 Fold cross validation}
\label{alg:10_fold_cross_valid}
\begin{algorithmic}[1]
\STATE The dataset is shuffled randomly
\STATE The dataset is split into 10 groups
\FOR{each data group d out of 10 groups } 
    \STATE 10\% of data from d is taken as test data
    \STATE 10\% of data from d is taken as verification data
    \STATE 80\% of data from d is taken as training data
    \STATE Our model is fitted on the training set and evaluate it on the test set
    \STATE The evaluation score is retained and the model is discarded 
\ENDFOR
\STATE The performance of the model is averaged using the sample of model evaluation scores
\end{algorithmic}
\end{algorithm}


==> Tex_Code/4.experiment/C.Result.analysis.tex <==
\subsection{Result Analysis}
\input{Tex_Code/4.experiment/performance_table}
\input{Tex_Code/4.experiment/bar_chart_performance_compare}

\begin{enumerate}
\item Performance of stylometric feature: 

We present the performance of stylometric feature along with traditional machine learning and deep learning algorithms in Table~\ref{performance-table-stylometric-feature}. From Table~\ref{performance-table-stylometric-feature}, we can see that deep learning algorithms like LSTM \& GRU performs better than traditional machine learning algorithms such as SVM \& NB. We have used stylometric features that can capture the writing style of different authors of both genders. LSTM and GRU models performs almost same in case of stylometric feature as GRU is a recently-developed variation of the long short-term memory~\cite{agarap_abien}. SVM outperforms the NB model because SVM model with stylometric feature can linearly separates data of two classes. Again, LSTM having feedback connections can process entire sequence of data. Thus LSTM with stylometric feature outperforms traditional machine learning algorithm like SVM and NB. 

\item Performance of word embedding feature:

We have experimented using word embedding as feature with both deep learning and traditional machine learning algorithms. The performance comparison is  
noted down in Table~\ref{performance-table-embedding-feature}.  The performance LSTM with word embedding feature outperforms SVM and NB model. LSTM can keep previous states. Also, we have used Word2vec~\cite{mikolov_kai} which can generate word vector based on the context. Thus the performance of LSTM model in cobination with word embedding feature is better than traditional machine learning model.    
% 
\item Performance of TF-IDF feature: 


The performance of TF-IDF feature vector in ccordance with deep learning algorithm like LSTM, GRU and traditional machine learning algorithm such as SVM, NB is presented in Table~\ref{performance-table-tfidf-feature}. Here, NB model outperforms SVM, GRU, and LSTM model.TF-IDF feature representation, a bag of words(BOW) feature,  is used to assign weight to a word based on the number of times it appears in the text.As NB model predicts the output class based on probability of the given vector, so NM model with TF-IDF feature outperforms other model. The highest accuracy is 77.82\% got by NB model with TF-IDF feature. 

  \item Performance among different models:    


  We present the performance of different machine learning model associated with the feature vector in table~\ref{performance-table-different-model}. This table is a summarising table of Table~\ref{performance-table-stylometric-feature},~\ref{performance-table-embedding-feature}, and~\ref{performance-table-tfidf-feature}. We have presented the performance result of Table~\ref{performance-table-stylometric-feature},~\ref{performance-table-embedding-feature}, and~\ref{performance-table-tfidf-feature} in Fig~\ref{performance_compare_model_feature}. Accuracy comparison is shown in Fig. ~\ref{accuracy_compare_model_feature} and F1 score is shown in Fig.~\ref{f1_score_compare_model_feature}. If we take best performance of machine learning algorithm in terms of feature, then we will get Table~\ref{performance-table-different-model}. From Table~\ref{performance-table-different-model}, we can see that traditional model like SVM and NB outperforms deep learning model such as LSTM. LSTM with word embedding feature is slightly better than GRU with the stylometric feature. This is expected as embedding feature captures the contexts of text where as the stylometric feature captures the authors writing style. SVM is slightly better than NB in terms of accuracy, since the NB works based on simpler computation of text frequency to compute the posterior probability of each classes. On the other hand, SVM works based on computation of hyperplane equation which separates data into classes perfectly~\cite{Kusumawati_2019}. The highest accuracy and F1-score got by our proposed methods are 76.28\% and 85.91\% accordingly.
  
\item Word Vector Performance: 


We have employed both trainable and non-trainable weights to CBOW and SG architectures of word2vec model. The performance of the trainable and nontrainable weight scheme to CBOW and SG is listed in Table ~\ref{performance-table-word2vec-model}. Continuous Bag of Words(CBOW) model gives the best accuracy and F1 score in all cases. Trainable weight initialization of embedding layer in case of CBOW architecture is better than static weight initialization. The reason behind CBOW is slightly superior to skip-gram is probably because the dataset may contain more frequently occurring words rather than sparse or infrequent words. CBOW architecture predicts most probable word (most frequently occurring word) given a context as opposed to infrequent or rare word in case of Skip-gram. Again, if we allow to update embedding of words in embedding layer, then it can not maintain contextual information. That is why, non-trainable Continuous Bag of Words model performs better than trainable Continuous Bag of Words. 
 

\item Language Specific Performance

Gender identification from text is a well studied problem in different language. We have shown the performance of gender identification from the text of various languages in table ~\ref{performance-measure-on-specific-language}. From Table ~\ref{performance-measure-on-specific-language}, it is evident that research on the English language~\cite{Cheng_Na} by traditional machine learning model gives the highest accuracy. For the deep learning model, research~\cite{Bsir_zrigui} on the Arabic language gives the best accuracy. For the F1-score, research~\cite{sboev_rybka} on the Russian language gives the best sensitivity score in both traditional and deep learning models. 2\textsuperscript{nd} highest F1-score is got by research on Bangla language performed by our work. We can explain the differences in performances of author gender identification from a text in different languages in terms of data, feature selection, and machine learning model. The comparison on research of different languages is shown in Table~\ref{method-compare-on-specific-language}. Stylometric features, TF-IDF and other variants of BOW feature can accurately detect writing style and pattern of author. Again, researchers ~\cite{T_YILDIZ} have shown that neural network architectures cannot show better performance than traditional ML methods with regard to author gender identification.


As researchers for English language~\cite{Cheng_Na} and Arabic language~\cite{shalabi_kanaanbt} have used stylometric features with traditional machine learning model, so the research on the English language and Arabic language has the highest and 2nd  highest accuracy 83\% and 80.4\% respectively. Then comes another research~\cite{Bsir_zrigui} on Arabic which has the 3rd highest accuracy. In this work, the researchers have used variant of BOW features. Deep learning model, Bi-GRU is used as machine learning model classifier in this language. Researchers in ~\cite{T_YILDIZ} shown that traditional machine learning model like SVM and NB works better than deep learning model like CNN and RNN model. Here, Word2vec, GloVe, TF-IDF etc. are used as feature vector. NB model combined with TF-IDF feature vector provides the maximum F1-score in this work. 

% For identification of author gender from English text, researchers~\cite{Cheng_Na} have taken two types of dataset: one from newspaper and another from email dataset of a company. They have used 5 types of stylometric features: character based features, word based features, syntactic features, structural features and functional word features. Corresponding machine learning models are Decision tree, Logistic Regression and Support Vector Machine. These models are from traditional machine learning models. \endgraf 

% For Arabic, researchers~\cite{Bsir_zrigui} have taken  Facebook comments and Twitter dataset. They have used Arabic Lexical features, Arabic n-grams, Arabic syntax features, Arabic character frequencies, and  Bag of smileys as features. These features are variant of 

 
  
\item Performance of deep learning model vs traditional machine learning model:


The comparison of performance between traditional machine learning(SVM, NB) model and the deep learning(LSTM) model is presented in Table~\ref{performance-table-different-model}. Foe feature representation, we have compared both traditional representations such as TF/IDF which is a variant of BOW and embedding representations such as Word2vec. Even though the drawback of BOW approach is the the curse of dimensionality, the BOW approach has still the power to solve solve our gender problem. TF/IDF vectorizer performs better than Context based Word2vec vectorizer approach. From Table~\ref{performance-table-different-model}, we can see that traditional ML models show better performance than neural network model. Widely used algorithms such as SVM and NB have proved to be efficient and successful for author gender identifications. SVM algorithm can segregate text according to gender by creating decision boundary. 
We have used linear decision boundary. Naive Bayes classifiers categorize text data based on strong independence assumptions between the features. On the other hand, neural network model such as LSTM categorize data based on weights which seems to be under-performed in our study. This result is consistent with research work ~\cite{sboev_rybka,T_YILDIZ}

\end{enumerate}


==> Tex_Code/4.experiment/bar_chart_performance_compare.tex <==

\begin{figure*}[!tbp]
       \centering
\begin{subfigure}[t]{0.45\textwidth}
\pgfplotstableread[col sep=comma]{
  X,  Y1, Y2, Y3
LSTM, 74.91, 75.62, 73.46
GRU,  74.91, 73.98, 73.71
SVM,  72.68, 74.87, 77.56
NB,   63.02, 74.23, 77.82
    }\mydata

    \begin{tikzpicture}
    \begin{axis}[
        height=75mm, width=90mm,
%
        bar width=0.17,
        ybar=2pt,
        enlarge x limits={abs=0.5},
        ymin=50,
        ymax=100,
        ytick distance=10,
        yticklabel style={font=\small},
        yticklabel=\pgfmathprintnumber{\tick}\,$\%$,
        ylabel={Performance in Percentage},
        xlabel={Machine Learning Model},
        xtick=data,
        xticklabels from table={\mydata}{X},
        nodes near coords,
        nodes near coords style={font=\tiny,             /pgf/number format/.cd,
        precision=1,
        zerofill,},
        legend style={legend pos=north east,cells={anchor=west},
        font=\footnotesize, }
    ]
\addplot table [x expr=\coordindex,y=Y1]{\mydata};
\addplot table [x expr=\coordindex,y=Y2]{\mydata};
\addplot table [x expr=\coordindex,y=Y3]{\mydata};
\legend{Stylometric Feature, Word Embedding Feature, TF-IDF Feature}    \end{axis}
    \end{tikzpicture}
\caption{Accuracy Comparison} \label{accuracy_compare_model_feature}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.45\textwidth}
\pgfplotstableread[col sep=comma]{
  X,  Y1, Y2, Y3
LSTM, 80.23, 81.21, 84.09
GRU,  80.24, 79.92, 84.02
SVM,  78.85, 85.63, 86.93
NB,   68.34, 85.18, 87.18
    }\mydata

    \begin{tikzpicture}
    \begin{axis}[
        height=75mm, width=90mm,
%
        bar width=0.15,
        ybar=2pt,
        enlarge x limits={abs=0.5},
        ymin=60,
        ymax=100,
        ytick distance=10,
        yticklabel style={font=\small},
        yticklabel=\pgfmathprintnumber{\tick}\,$\%$,
        ylabel={Performance in Percentage},
        xlabel={Machine Learning Model},
        xtick=data,
        xticklabels from table={\mydata}{X},
        nodes near coords,
        nodes near coords style={font=\tiny,             /pgf/number format/.cd,
        precision=1,
        zerofill,},
        legend style={legend pos=north east,cells={anchor=west},
        font=\footnotesize, }
    ]
\addplot table [x expr=\coordindex,y=Y1]{\mydata};
\addplot table [x expr=\coordindex,y=Y2]{\mydata};
\addplot table [x expr=\coordindex,y=Y3]{\mydata};
\legend{Stylometric Feature, Word Embedding Feature, TF-IDF Feature}    \end{axis}
    \end{tikzpicture}
\caption{F1 Score Comparison}
\label{f1_score_compare_model_feature} 
\end{subfigure}
\caption{Performance comparison of different machine learning models with feature}
  \label{performance_compare_model_feature}
\end{figure*}



==> Tex_Code/4.experiment/performance_table.tex <==


 
\begin{table*}[t]
 \caption{Performance measure for Stylometric Feature: 
}
\label{performance-table-stylometric-feature}
\begin{tabularx}{\textwidth}{@{}l*{2}{C}c@{}} 
\toprule
Model & Feature Vector & Accuracy & F1-score \\
\midrule
LSTM & Styoletric Feature & 74.91\% & 80.23\% \\ 
GRU & Styoletric Feature & 74.91\% & 80.24\%  \\ 
SVM & Styoletric Feature & 72.68\% & 78.85\% \\ 
NB & Styoletric Feature & 63.02\% & 68.34\% \\ 
\bottomrule
\end{tabularx} 
\end{table*}

\begin{table*}[t]
 \caption{Performance measure for Word Embedding Feature: 
}
\label{performance-table-embedding-feature}
\begin{tabularx}{\textwidth}{@{}l*{2}{C}c@{}} 
\toprule
Model & Feature Vector & Accuracy & F1-score \\
\midrule
LSTM & Word Embedding Feature & 75.62\% & 81.21\% \\ 
GRU & Word Embedding Feature & 73.98\% & 79.92\%  \\ 
SVM & Word Embedding Feature & 74.87\% & 85.63\% \\ 
NB & Word Embedding Feature & 74.23\% & 85.18\% \\ 
\bottomrule
\end{tabularx} 
\end{table*}

\begin{table*}[t]
 \caption{Performance measure for TF-IDF Feature: 
}
\label{performance-table-tfidf-feature}
\begin{tabularx}{\textwidth}{@{}l*{2}{C}c@{}} 
\toprule
Model & Feature Vector & Accuracy & F1-score \\
\midrule
LSTM & TF-IDF Feature & 73.46\% & 84.09\% \\ 
GRU & TF-IDF Feature & 73.71\% & 84.02\%  \\ 
SVM & TF-IDF Feature & 77.46\% & 86.93\% \\ 
NB & TF-IDF Feature & 77.82\% & 87.18\% \\ 
\bottomrule
\end{tabularx} 
\end{table*}

\begin{table*}[t]
 \caption{Performance measure for Different Models}
\label{performance-table-different-model}
\begin{tabularx}{\textwidth}{@{}l*{2}{C}c@{}} 
\toprule
Model & Feature Vector & Accuracy & F1-score \\
\midrule
 LSTM & Word embedding Feature & 75.62\% & 81.21\%  \\ 
 GRU & Styoletric Feature & 74.91\% & 80.24\% \\ 
SVM & TF-IDF Feature & 77.56\% & 86.93\% \\ 
NB & TF-IDF Feature & 77.82\% & 87.18\% \\ 
\bottomrule
\end{tabularx} 
\end{table*}

\begin{table*}[t]
 \caption{Performance measure for Word Vector Model}
\label{performance-table-word2vec-model}
\begin{tabularx}{\textwidth}{@{}l*{10}{C}c@{}}
\toprule
Vectorization model & Accuracy & F1-Score\\
\midrule
Continuous Bag of Words (Trainable) &  75.13\% & 79.92\% \\ 
Continuous Bag of Words (Non-Trainable) & 75.62\% & 81.21\%\\ 
Skip-Gram(Trainable) & 74.74\%  & 79.8\% \\ 
Skip-Gram(Non-Trainable) & 75.62\% & 81.2\% \\ 
\bottomrule
\end{tabularx}
\end{table*}


 \begin{table*}
    \setcellgapes{3pt}
    \makegapedcells
\caption{Performance measure on specific language }
\label{performance-measure-on-specific-language}
\begin{tabularx}{\textwidth}{ | *{6}{C|} }
  \hline
\multirow{2.5}{=}{ Language }
    &   \multirow{2.5}{=}{ Proposed By }
        &   \multicolumn{2}{c|}{ Accuracy } 
            &   \multicolumn{2}{c|}{ Sensitivity }      \\
    \cline{3-6}
    &   & Traditional  & Deep Learning & Traditional & Deep Learning    \\ 
    \hline
   Arabic & ~\cite{shalabi_kanaanbt}  & 80.4\%  & 76.6\% & 80.4\% & 76.3\% - -    \\
    \hline
   Arabic & ~\cite{Bsir_zrigui} & - - - - & 79\%  & - - - - & - - - -    \\
    \hline
    English & ~\cite{Cheng_Na}  & 82.23\%  & - - - - & - - - - & - - - -    \\
    \hline
    Russia & ~\cite{sboev_rybka}  & 77\%  & 76\% & 91\% & 89\%  \\
    \hline
    Turkish & ~\cite{T_YILDIZ}  & - - -  & - - - & 79\% & 69\%  \\
    \hline
    Bangla &  own & 77.82\%  & 76.03\% & 87.18\% & 81.21\%   \\
    \hline
\end{tabularx}
    \end{table*}
    

\begin{table*}
\setcellgapes{3pt}
\makegapedcells
\caption{Method compare on research of specific language}
\label{method-compare-on-specific-language}
\begin{tabularx}{\textwidth}{ | *{7}{C|} }
  \hline
  Language &  Proposed by &  Dataset &  Feature &  Model &  Model Type &  Accuracy/F1-score \\ 
  \hline 
  Arabic & ~\cite{shalabi_kanaanbt}  & News Website Article &
  Character based, word based, syntactic, semantic \& functional word
  & BN, NB, Logis, ANN, SGD, SLogis, SVM, KNN, DT, JRip, OneR, PART, J48, RF  & Traditional & Accuracy - 80.4\%   \\
    \hline
   Arabic & ~\cite{Bsir_zrigui} & Facebook comments and Twitter text
& Lexical features, n-grams, syntax features, character frequencies, Bag of smileys, Arabic stop words
& Bi-Gated Recurrent Unit Layer & Deep Learning &  Accuracy- 79\%  \\
    \hline
    English & ~\cite{Cheng_Na}  & Online multimedia newspaper, Email dataset of Company & Character-based, Word-based, Syntactic, and Structural features, Function words
 & SVM, Adaboost Decision Tree, Logistic Regression   
 & Traditional &Accuracy -  83\%  \\
    \hline
    Russia & ~\cite{sboev_rybka} &  Russian pre-existing corpus
 & Morphological features, Syntactical parameters, Derivative coefficients, No. of words pertaining emotion & Gradient Boosting,
 Adaptive Boosting, 
ExtraTrees, Random Forest,
PNN, Support Vector Machine, CNN, LSTM
 & Both traditional \& deep learning & Traditional model accuracy- 77\%,\newline Deep learning model accuracy - 76\%\\
    \hline
     Turkish & ~\cite{T_YILDIZ}  & Turkish news websites  & Uni-gram, Bi-gram, TF-IDF, Word2vec, GloVe, Doc2vec & KNN, NB, LR, SVM, SGD, Decision Tree, Random Forest, Multi-Layer Perceptron, CNN, RNN & Both traditional \& deep learning & Traditional mode F1-score - 78\% \& Deep learning F1-score - 69\%  58\%  \\
    \hline
Bangla &  own & User Status from Facebook Group & Character based, word based, syntactic, semantic, functional word \& word embedding using word2vec model & LSTM, SVM, NB & Both traditional \& deep learning & Traditional - 76.28\%,\newline Deep learning- 76.03\%\\
    \hline
  
 \end{tabularx}
\end{table*}

==> Tex_Code/6.acknowledge/acknowledgement.tex <==


The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

==> Tex_Code/7.references/nokol.tex <==

\bibitem{b1} Corney, M., Vel, O. d., Anderson, A., and Mohay, G., “Gender-preferential text mining of e-mail discourse,” in Computer Security Applications Conference(CSAC), Las Vegas, USA, Dec 9-13, 2002.

\bibitem{b2} Keselj, V., Peng, F., Cercone, N., and Thomas, C., “N-gram-based author profiles for authorship attribution,” in Pacific Association for Computational Linguistics, Halifox, Canada, Aug 22-25,2003.

\bibitem{b3} Rangel, F., Rosso, P., Potthast, M., and Stein, B., “Overview of the 5th author profiling task at pan 2017: Gender and language variety identification in twitter,” in Notebook for PAN at CLEF, Dublin, Ireland, Sept 11-14 , 2017.
\bibitem{b4} Vollenbroek, M. B. o., Carlotto, T., Kreutz, T., Medvedeva, M., Pool, C., Bjerva, J., Haagsma, H., and Nissim, M., “Content-centric age and gender profiling,” in Notebook for PAN at CLEF, Évora, Portugal, Sept 05-08 , 2016.
\bibitem{b5} Lim, W.-Y., Goh, J., and Thing, V. L. L., “Content-centric age and gender profiling,” in Notebook for PAN at CLEF, Valencia, Spain, Sept 23-26, 2013.
\bibitem{b6} Rosenthal, S., Agarwal, A., and McKeown, K., “Columbia nlp: Sentiment detection of sentences and subjective phrases in social media,” in Semantic Evaluation (SemEval), Dublin, Ireland, Aug 23-24, 2014.
\bibitem{b7} Sboev, A., Litvinova, T., Voronina, I., Gudovskikh, D., and Rybka, R., “Deep learning network models to categorize texts according to author’s gender and to identify text sentiment,” in Computational Science and Computational Intelligence (CSCI), Las Vegas, USA, Dec 15-17, 2016.
\bibitem{b8} lsmearat, K., Al-Ayyouba, M., Al-Shalabi, R., and Kanaanbt, G., “Author gender identification from arabic text,” Journal of Information Security and Applications , vol. 35, no. 8, pp. 85–95, 2017.
\bibitem{b9} Bsir,  B. and Zrigui,  M.,  “Enhancing deep learning gender identification with gated recurrent units architecture in social text,” Computación y Sistemas , vol. 22, no. 3, pp. 757–766, 2018.
\bibitem{b10} Rahman, S. M., Kabir, F. M., Kabir, F. M., and Huda, N. M., “Automatic gender identification system for bengali speech,” in Electrical Information and Communication Technologies (EICT), Khulna, Bangladesh, Dec 10-12 , 2015.
\bibitem{b11} Tripto, N. I., and Ali, M. E. “Detecting Multilabel Sentiment and Emotions from Bangla YouTube Comments,” in International Conference on Bangla Speech and Language Processing (ICBSLP), Sylhet, Bangladesh, Sept 21-22 , 2018.

==> Tex_Code/7.references/references.tex <==
\printbibliography

==> Tex_Code/resource/table/3.C.stylo.table.tex <==

\begin{table*}[hp]
\caption{Stylometric Features}
\label{stylometric-features-table}
    \centering
    \begin{tabularx}{\textwidth}{| X | X | X |}
        \hline
       
        \multicolumn{3}{|c|}{Character Based Lexical Features} \\
        \hline
        Feature Name & Feature Count & Feature Description \\ 
        \hline
        Total characters $ \implies$ C   & $F_1$ & Alphabet, digits, special characters\\
        \hline
        Total number of letters/C & $F_2$ &  অ -  ঁ  \\\hline
        Total number of digits/C & $F_3$ & ০-৯ \\\hline
        Total number of white-space characters/C & $F_4$ & white sapce  \\\hline
        Total number of tab space characters/C & $F_5$ & tab space \\\hline
        Total number of elongation characters/C & $F_6$ & total word that pronounced as long \\\hline
        Total number of dependent vowel characters/C & $ F_7  \cdots F_{17} $ &  া , ি , ী , ◌ু ,  ◌ূ , ◌ৃ , ◌ৄ ,  ে ,  ৈ  \\ \hline
        Total number of special characters/C & $ F_{18}  \cdots F_{41} $ &  
         «,  », \$, \%, \&, *, (, ), $>$, $<$, \{, \}, [, ], \_, +, -, =, \^ , \/,$ \backslash\backslash $, \textasciitilde, |          
        \\ \hline
        Total number of individual characters/C & $ F_{42}  \cdots F_{91} $ & অ - ঁ  \\
        \hline
        \multicolumn{3}{|c|}{Word Based Lexical Features} \\
        \hline
        Feature Name & Feature Count & Feature Description \\ 
        \hline
        Total number of words & $F_{92}$  & Total number of all words in the text  \\ \hline 
        Average word length & $F_{93}$ & The average number of characters per word \\ \hline
        Total Unique words & $F_{94}$ & Words that appear once in a text  \\ \hline
        Hapex legomena & $F_{95}$ & Words that occurs only one \\ \hline
        Hapax Dislegomena & $F_{96}$ & Words that occurs only twice \\ \hline
        Total no. of Short words & $F_{97}$ & 1-3 character words \\ \hline
        Total no. of Long words & $F_{98}$ & Words longer than 6 characters  \\ \hline
        Word length frequency distribution & $F_{99} \cdots F_{114} $ & word length from 0 to 15  \\ \hline
        Yules K measure & $F_{115}$ & Measure of vocabulary richness  \\ \hline
        Total Digit word & $F_{116}$ & words that have digits \\ \hline
        Total Consecutive occurrence & $F_{117}$ & no of words with 3 consecutive duplicate characters \\ \hline 
        
         \multicolumn{3}{|c|}{Syntactic Features} \\
        \hline
        Feature Name & Feature Count & Feature Description \\ 
        \hline
        Total single quotes/C   & $F_{118}$ & ' \\
        Total comma/C & $F_{119}$ & ,  \\
        Total periods/C & $F_{120}$ & . \\
        Total colons/C & $F_{121}$ & :  \\
        Total semi colons/C & $F_{122}$ & ; \\
        Total question marks/C & $F_{123}$ & ? \\
        Total exclamation marks/C & $F_{124}$ & ! \\
        Total double quotes/C & $F_{125}$ &  "  \\ 
        \hline 
        
            
\multicolumn{3}{|c|}{Structural Features} \\
\hline
        Feature Name & Feature Count & Feature Description \\ 
        \hline
        Total number of lines & $F_{126}$ & line splitted by । \\
        Total number of paragraphs & $F_{127}$ & in the case of pressing enter \\
        Total number of sentences & $F_{128}$ &  \\
        Total number of blank lines & $F_{129}$ & in the case of pressing enter \\
        Total number of non blank lines & $F_{130}$ & \\
        Total length of non blank lines & $F_{131}$ & \\
        Average length of non blank lines & $F_{132}$ & \\
        Average number of words per sentence & $F_{133}$ & \\
        Average number of words per paragraph & $F_{134}$ & \\
        Average number of character per sentence & $F_{135}$ & \\
        Average number of  character per paragraph & $F_{136}$ &  \\
        \hline  
        
        \multicolumn{3}{|c|}{Content Specific Features} \\
\hline
Feature Name & Feature Count & Feature Examples \\ 
\hline
        Total economic phrases & $F_{137}$ & রাজ্য তহবিল (State funds), কোম্পানি (Company), বিনিয়োগ(Investment) \\
         \hline 
        Total policy phrases & $F_{138}$ & রাষ্ট্রদূত(Ambassador), বিশৃঙ্খল(Chaotic), যত্ন(Care) \\
         \hline 
        Total Social phrases & $F_{139}$ & নারী অধিকার(Women's rights), বংশ(race), যুব গ্রুপ(youth group) \\
         \hline 
        Total Sports phrases & $F_{140}$ & খেলা(Sports), ফুটবল(Football), পদক(Medal)\\
         \hline 
        Total Negative phrases & $F_{141}$ & পরিত্যাগ করা(abandon), ঘৃণা(hatred), পলায়ন(escape)\\
        \hline 
    \end{tabularx}
\end{table*} 

==> Tex_Code/resource/table/3.c.stylo.translate.tex <==

\begin{table*}[htp]
\caption{Examples of Arabic and Translated Bangla \& English Words}
\label{arabic-translated-bangla}
    \centering
    \begin{tabularx}{\textwidth}{| X | X | X |  X |  X |}
        \hline
        Economy & Policy & Social & Sport & Negative \\ 
        \hline 
\arab{﻿اموال الدوله } & \arab{إساءة استخدام القوة} & \arab{ثقافات} & \arab{﻿كره القدم} & \arab{مهجور}\\ 
{\beng রাজ্য তহবিল } 
   & {\beng ক্ষমতার অপব্যবহার} & {\beng সংস্কৃতি} & {\beng ফুটবল} & {\beng পরিত্যক্ত} \\
State funds & Abuse of power & Culture & Football & Abandoned \\ 
        \hline 
        \arab{بنك} &\arab{وزير بالوكالة } & \arab{قبيله}& \arab{رياضه} & \arab{غير طبيعي}\\
        {\beng ব্যাংক }  & {\beng  ভারপ্রাপ্ত মন্ত্রী }    & {\beng উপজাতি} & {\beng খেলা}&  অস্বাভাবিক \\
     Bank & Minister in charge & Tribe & Sport & Abnormal
        \\
        \hline
        \arab{انهيار اقتصادي} & \arab{لجنة استشارية}  & \arab{طالبات المدارس} & \arab{ملعب} & \arab{إلغاء}\\
     {\beng অর্থনৈতিক পতন} & {\beng উপদেষ্টা কমিটি} & {\beng স্কুল} &  {\beng স্টেডিয়াম }& {\beng বাতিল } \\
      Economic Fall & Advisory Committee & School & Stadium &  Cancel
     \\
        \hline
        \arab{شركات} & \arab{مداولة} & \arab{اسره}& \arab{مباريات}& \arab{مفاجئ}\\
     কোম্পানি  & {\beng পরামর্শ} & {\beng পরিবার} & {\beng গেম} & {\beng আকস্মিক} \\
    Company & Advice & Family & Game & Sudden
     \\
        \hline
    \end{tabularx}
\end{table*} 
